A Virtual Frame Buffer Abstraction for Parallel Rendering of Large Tiled Display Walls

We present dw2, a flexible and easy-to-use software infrastructure for interactive rendering of large tiled display walls. Our library represents the tiled display wall as a single virtual screen through a display "service", which renderers connect to and send image tiles to be displayed, either from an on-site or remote cluster. The display service can be easily configured to support a range of typical network and display hardware configurations; the client library provides a straightforward interface for easy integration into existing renderers. We evaluate the performance of our display wall service in different configurations using a CPU and GPU ray tracer, in both on-site and remote rendering scenarios using multiple display walls

==> Makefile <==
CONTENT=ospDisplayWall
BIBLIOGRAPHY=$(wildcard *.bib)
ALLTEXFILES=$(wildcard *.tex *.tex)
ALLFIGS=$(wildcard png/*)
LATEX_ARGS=-halt-on-error --shell-escape

all: $(CONTENT).pdf

$(CONTENT).pdf: $(ALLTEXFILES) $(ALLFIGS) $(BIBLIOGRAPHY)
	pdflatex $(LATEX_ARGS) $(CONTENT)

$(CONTENT)-compressed.pdf: final
	gs -sDEVICE=pdfwrite -o $@ \
		-dPDFSETTINGS=/prepress \
		-dDownsampleColorImages=true \
		-dDownsampleGrayImages=true \
		-dDownsampleMonoImages=true \
		-dColorImageResolution=600 \
		-dDoThumbnails=false \
		-f $(CONTENT).pdf

.PHONY: final
final: $(CONTENT).pdf
	bibtex $(CONTENT)
	pdflatex $(LATEX_ARGS) $(CONTENT)
	pdflatex $(LATEX_ARGS) $(CONTENT)

.PHONY: compress
compress: ${CONTENT}-compressed.pdf

.PHONY: update_check
update_check:
	wget https://raw.githubusercontent.com/erich666/chex_latex/master/chex_latex.pl \
		-O ./scripts/chex_latex.pl

.PHONY: check
check:
	perl ./scripts/chex_latex.pl $(ALLTEXFILES)

.PHONY: clean
clean:
	rm -f *.aux *.bbl *.blg *.dvi *.lbl *.log $(CONTENT).pdf \
		$(CONTENT)-final.pdf *.ps *.brf

